Quality and Quantity: Unveiling a Million High-Quality Images for Text-to-Image Synthesis in Fashion Design

The fusion of AI and fashion design has emerged as a promising research area. However, the lack of extensive, interrelated data on clothing and try-on stages has hindered the full potential of AI in this domain. Addressing this, we present the Fashion-Diffusion dataset, a product of multiple years' rigorous effort. This dataset, the first of its kind, comprises over a million high-quality fashion images, paired with detailed text descriptions. Sourced from a diverse range of geographical locations and cultural backgrounds, the dataset encapsulates global fashion trends. The images have been meticulously annotated with fine-grained attributes related to clothing and humans, simplifying the fashion design process into a Text-to-Image (T2I) task. The Fashion-Diffusion dataset not only provides high-quality text-image pairs and diverse human-garment pairs but also serves as a large-scale resource about humans, thereby facilitating research in T2I generation. Moreover, to foster standardization in the T2I-based fashion design field, we propose a new benchmark comprising multiple datasets for evaluating the performance of fashion design models. This work represents a significant leap forward in the realm of AI-driven fashion design, setting a new standard for future research in this field.

==> sec/7_eth.tex <==
\section{Ethics Statement}
\label{eth}

In this section, we discuss three primary ethical considerations regarding our Fashion-Diffusion dataset.

\begin{itemize}%[topsep=3pt, itemsep=2pt, parsep=0pt, leftmargin=10pt]
  \item \textbf{Copyright.}
  When using our text-to-image generation website, all users consent to our privacy policy and data usage agreement.
  This includes academic utilization and the dissemination of any content hosted on the server, such as anonymized prompts, images, and user iterations.

  \item \textbf{Privacy.}
  We've ensured that all user data in the Fashion-Diffusion dataset, including usernames and other private details, has been anonymized.
  It is worth noting that while rare, there is a possibility that certain prompts could contain sensitive information. But, this is uncommon because our website has strict rules against writing personal information in the prompts, and has professional detectors to eliminate any violative content as well.
  \item \textbf{Potential Harm.}
  Although we have built strong detectors to filter out inappropriate material on our website, there remains a potential for occasional instances of NSFW ? (Not Safe for Work) content to emerge in Fashion-Diffusion dataset.

\end{itemize}

==> sec/_1.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics{figs/Figure1_left.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure*}

% We move to the main content: "1_intro.tex"
